RoboBrain: A Unified Brain Model for Robotic Manipulation from Abstract to Concrete

Recent advancements in Multimodal Large Language Models (MLLMs) have shown remarkable capabilities across various multimodal contexts. However, their application in robotic scenarios, particularly for long-horizon manipulation tasks, reveals significant limitations. These limitations arise from the current MLLMs lacking three essential robotic brain capabilities: Planning Capability, which involves decomposing complex manipulation instructions into manageable sub-tasks; Affordance Perception, the ability to recognize and interpret the affordances of interactive objects; and Trajectory Prediction, the foresight to anticipate the complete manipulation trajectory necessary for successful execution. To enhance the robotic brain's core capabilities from abstract to concrete, we introduce ShareRobot, a high-quality heterogeneous dataset that labels multi-dimensional information such as task planning, object affordance, and end-effector trajectory. ShareRobot's diversity and accuracy have been meticulously refined by three human annotators. Building on this dataset, we developed RoboBrain, an MLLM-based model that combines robotic and general multi-modal data, utilizes a multi-stage training strategy, and incorporates long videos and high-resolution images to improve its robotic manipulation capabilities. Extensive experiments demonstrate that RoboBrain achieves state-of-the-art performance across various robotic tasks, highlighting its potential to advance robotic brain capabilities.

==> sec/7_afford_and_traj.tex <==
\subsubsection{Trajectory}
\paragraph{Trajectory Representation}
The term \textbf{trajectory} in our work refers to the concept of \textit{2D visual traces}, as presented in \cite{gu2023rt}. These trajectories are similar to the \textit{2D waypoints} described in \cite{cheng2024empowering,kuang2024ram}. Our research emphasizes \textit{coarse trajectories} that capture spatial patterns in two-dimensional space, rather than focusing on complex and fine-grained states and actions. We define trajectory waypoints as a series of 2D coordinates representing the movement of the gripper (or end-effector, hand, etc.) throughout the process.

Formally, at time step $t$, the trajectory waypoints can be represented as:
\[
P_{t:N} = \{(x_i, y_i) \mid i = t, t + 1, \dots, N\}
\]
where $(x_i, y_i)$ denotes the $i$-th coordinate in the visual trace, and $N$ represents the total number of time steps in the episode.


\paragraph{Trajectory Finetuning}
Similar to visual grounding, we require MLLMs to predict a series of 2D coordinates on the image that represent trajectory waypoints. We use trajectory data from the dataset introduced in \cite{niu2024llarva}, which annotates numerous trajectories from a subset of Open X-Embodiment (OXE) \cite{o2023open}, using a custom-trained Detectron2 model. To ensure data quality, we apply the RANSAC algorithm \cite{fischler1981random} to remove outliers from the target waypoints. Given an observation image and specific task goals, such as \verb+pick apple from top drawer+, the model is tasked with predicting a sequence of trajectory waypoints that guide the robot in completing the task.

\subsubsection{Affordance}

\paragraph{Affordance Representation} In our paper, we define the affordance of objects as the area where the human hand makes contact with them. During interactions, humans instinctively engage with various objects within specific regions. We use the \textbf{bounding boxes} to represent affordances because, on one hand, most vision-language models own the ability of visual grounding, and fine-tuning based on this format is beneficial for affordances. On the other hand, bounding boxes provide a broader and more robust spatial representation; compared to point representations, bounding boxes can effectively convey the area within which the robot needs to operate, even with slight deviations. 

Consider an image $I$ consisting of multiple objects with their affordances: $O_i = \{A_{i}^{0}, A_{i}^{1}, ..., A_{i}^{N}\}$, where the $i$th object owns $N$ affordances. Besides, the format of affordance is defined as $\{l^{(x)}, l^{(y)}, r^{(x)}, r^{(y)}\}$, and $\{l^{(x)}, l^{(y)}\}$ means the top left corner coordinates of affordance, while $\{r^{(x)}, r^{(y)}\}$ means the bottom right corner coordinates.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/affordance.pdf}
    \caption{The prompt-aware affordance training sample.}
    \label{fig:affordance}
\end{figure}

\paragraph{Affordance Finetuning} Here, we explain how we construct the prompt-aware affordance training sample. Faced with various language questions, the label is different. For instance, as shown in Figure \ref{fig:affordance}, if we ask, \textit{Please add water to the teapot}, the annotation should identify the affordances corresponding to the lid. If the prompt is changed into, \textit{Please pour the tea from the teapot}, the label focuses on the teapot spout. Therefore, the instrction is vital to the localization of affordance. Eventually, we combine the above elements into a sample to form the \textbf{quadruple}:
\[
\{ I, \text{object}, \text{prompt}, \{l^{(x)}, l^{(y)}, r^{(x)}, r^{(y)}\} \}
\]
During the training process, we implement two optimizations: (1) a special token inspired by the [\texttt{CLS}] token, where we set up an affordance token to collect information from images and coordinates; (2) an appropriate mixture ratio of the training samples, where we find that suitable addition of general VQA during fine-tuning can help the model learn to understand how to bind text with affordance.

==> table/affordance.tex <==
\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.3} % Adjust row height
\setlength{\tabcolsep}{12pt}      % Adjust column spacing
\caption{Evaluation Results of Different Model Variants on 2D Trajectory Prediction}
\label{table:evaluation_trajectory}
\begin{tabular}{lccc}
\toprule
\textit{Model Variant}  & \textit{DFD} $\downarrow$ & \textit{HD} $\downarrow$ & \textit{RMSE} $\downarrow$ \\ \midrule
LLARVA                  & X.XXX                     & X.XXX                    & X.XXX                      \\
RoboBrain (Baseline      & X.XXX                     & X.XXX                    & X.XXX                      \\
+ Visual\_FT            & X.XXX                     & X.XXX                    & X.XXX                      \\
+ Start\_Points         & X.XXX                     & X.XXX                    & X.XXX                      \\
+ Max\_Points           & X.XXX                     & X.XXX                    & X.XXX                      \\
+ Spec\_Token           & X.XXX                     & X.XXX                    & X.XXX                      \\
+ Scratch               & X.XXX                     & X.XXX                    & X.XXX                      \\ \bottomrule
\end{tabular}
\end{table}
